Large Linear Multi-output Gaussian Process Learning

Gaussian processes (GPs), or distributions over arbitrary functions in a continuous domain, can be generalized to the multi-output case: a linear model of coregionalization (LMC) is one approach. LMCs estimate and exploit correlations across the multiple outputs. While model estimation can be performed efficiently for single-output GPs, these assume stationarity, but in the multi-output case the cross-covariance interaction is not stationary. We propose Large Linear GP (LLGP), which circumvents the need for stationarity by inducing structure in the LMC kernel through a common grid of inputs shared between outputs, enabling optimization of GP hyperparameters for multi-dimensional outputs and low-dimensional inputs. When applied to synthetic two-dimensional and real time series data, we find our theoretical improvement relative to the current solutions for multi-output GPs is realized with LLGP reducing training time while improving or maintaining predictive mean accuracy. Moreover, by using a direct likelihood approximation rather than a variational one, model confidence estimates are significantly improved.

==> representation.tex <==

\begin{tabular}{ccccccc}
  \toprule

  $D$ & $R$ & $Q$ & \textsc{cholesky} & \textsc{sum} & \textsc{bt} & \textsc{slfm}\\\midrule
 $ 2 $ & $ 2 $ & $ 10 $ & $ 43.62 $ & $ 3.72 $ & $ \textbf{0.89} $ & $ 3.71 $ \\ 
 $ 10 $ & $ 1 $ & $ 10 $ & $ 45.02 $ & $ 11.61 $ & $ 11.79 $ & $ \textbf{2.78} $ \\ 
 $ 10 $ & $ 10 $ & $ 1 $ & $ 14.25 $ & $ \textbf{0.24} $ & $ 1.74 $ & $ 0.42 $ \\ 
 \bottomrule 
 \end{tabular}
